Distributed mining of large scale remote sensing image archives on public computing infrastructures

Earth Observation (EO) mining aims at supporting efficient access and exploration of petabyte-scale space- and airborne remote sensing archives that are currently expanding at rates of terabytes per day. A significant challenge is performing the analysis required by envisaged applications --- like for instance process mapping for environmental risk management --- in reasonable time. In this work, we address the problem of content-based image retrieval via example-based queries from EO data archives. In particular, we focus on the analysis of polarimetric SAR data, for which target decomposition theorems have proved fundamental in discovering patterns in data and characterize the ground scattering properties. To this end, we propose an interactive region-oriented content-based image mining system in which 1) unsupervised ingestion processes are distributed onto virtual machines in elastic, on-demand computing infrastructures 2) archive-scale content hierarchical indexing is implemented in terms of a "big data" analytics cluster-computing framework 3) query processing amounts to traversing the generated binary tree index, computing distances that correspond to descriptor-based similarity measures between image groups and a query image tile. We describe in depth both the strategies and the actual implementations for the ingestion and indexing components, and verify the approach by experiments carried out on the NASA/JPL UAVSAR full polarimetric data archive. We report the results of the tests performed on computer clusters by using a public Infrastructure-as-a-Service and evaluating the impact of cluster configuration on system performance. Results are promising for data mapping and information retrieval applications.

==> discussions.tex <==
The aim of the present paper is to propose technological and algorithmic approaches to image mining in a \emph{big data} condition, 

The system is general, it allows fast searches basing on a hierarchical algorithm and uses Euclidean distances for retrieving contents that best match user queries.
$K$ means is suboptimal for binary space partitioning. A different approach would consist of choosing the optimal space partitioning, in terms of estimating the optimal number of clusters, at each node of the tree.
Due to the Euclidean distance measure adopted in the clustering method underlying the indexing mechanism, another possible weakness comes out. Indeed, it could be properly observed that such measure does not fit well with the nature of the features extracted from the polarimetric SAR images, i.e. histograms. During the ingestion phase, data point signatures are reshaped in one-dimensional vectors, thereby losing the "spatial" information contained in multidimensional histograms. Non-Euclidean distance measures are more suitable to quantify the difference between two probability distributions. Kullback-Leibler divergence [kullback info theory] and Earth Mover's Distance are possible choices (check!).

\textcolor{red}{Leggi Debatty04-par3. Discute del problema del k-means che deve salvare risultati su hdfs}.

\textcolor{red}{PARLARE DELLA SCELTA ARTICOLO FRANCESI}
Talk about network traffic.
Introdurre prima il concetto di indice costruito con albero (spiegare come avviene la ricerca, quindi dire che ci sono diversi modi per costruirlo, per esempio basati su ANN [Tobin06] ecc...)
Problema nel generare un indice per Terabyte scale data. Sistemi come Geoiris non fanno caso a questa richiesta, giustificandosi col termine "offline operations" [Klaric proc06]


Although developed for polarimetric SAR data, the system schema is general and can be further extended to include data from other sensor, thereby allowing efficient searching across heterogeneous  geospatial  repositories.  
In  particular,  an application to mine full Sentinel-1 archives can be devised by considering a quasi-complete description of the radar signal in  terms  of  textural  and  shape  descriptors  as  well  as  more advanced  descriptions  for  metric  resolution  data  based  on 
signal  decomposition  in  fractional  frequency  domains~\cite{walessa2000model,singh2013sar}.

Dire che è possibile fare analisi temporali.


